Conditional Contextual Refinement (CCR)

Contextual refinement (CR) is one of the standard notions of specifying open programs. CR has two main advantages: (i) (horizontal and vertical) compositionality that allows us to decompose a large contextual refinement into many smaller ones enabling modular and incremental verification, and (ii) no restriction on programming features thereby allowing, e.g., mutually recursive, pointer-value passing, and higher-order functions. However, CR has a downside that it cannot impose conditions on the context since it quantifies over all contexts, which indeed plays a key role in support of full compositionality and programming features. In this paper, we address the problem of finding a notion of refinement that satisfies all three requirements: support of full compositionality, full (sequential) programming features, and rich conditions on the context. As a solution, we propose a new theory of refinement, called CCR (Conditional Contextual Refinement), and develop a verification framework based on it, which allows us to modularly and incrementally verify a concrete module against an abstract module under separation-logic-style pre and post conditions about external modules. It is fully formalized in Coq and provides a proof mode that combines (i) simulation reasoning about preservation of sideffects such as IO events and termination and (ii) propositional reasoning about pre and post conditions. Also, the verification results are combined with CompCert, so that we formally establish behavioral refinement from top-level abstract programs, all the way down to their assembly code.

==> coq/abs.tex <==
\begin{coqdoccode}
\coqdocnoindent
\coqdockw{Variant} \coqdocvar{APCE}: \coqdockw{Type} \ensuremath{\rightarrow} \coqdockw{Type} := \ensuremath{|} \coqdocvar{APC}: \coqdocvar{APCE} \coqdocvar{unit}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Definition} \coqdocvar{absE} := \coqdocvar{APCE} +' \coqdocvar{emsE}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Record} \coqdocvar{abs}: \coqdockw{Type} := \coqdocvar{mk\_abs} \{\coqdoceol
\coqdocindent{1.00em}
\coqdocvar{mn}: \coqdocvar{string};\coqdoceol
\coqdocindent{1.00em}
\coqdocvar{functions\_friend}: \end{coqdoccode}
\begin{coqdoccode}
 \coqdocvar{string} \end{coqdoccode}
\hspace{-1pt}$\fpfn{}$\hspace{-5pt} \begin{coqdoccode}
 \coqdocvar{function} \coqdocvar{absE};\coqdoceol
\coqdocindent{1.00em}
\coqdocvar{functions\_context}: \coqdocvar{string} \end{coqdoccode}
\hspace{-1pt}$\fpfn{}$\hspace{-5pt} \begin{coqdoccode}
 \coqdocvar{function} \coqdocvar{absE};\coqdoceol
\coqdocindent{1.00em}
\coqdocvar{initial\_st}: \coqdocvar{Any};\coqdoceol
\coqdocnoindent
\}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Definition} \coqdocvar{rProp} := \coqdocvar{Σ} \ensuremath{\rightarrow} \coqdockw{Prop}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Record} \coqdocvar{spec}: \coqdockw{Type} := \coqdocvar{mk\_spec} \{\coqdoceol
\coqdocindent{1.00em}
\coqdocvar{meta}: \coqdockw{Type};\coqdoceol
\coqdocindent{1.00em}
\coqdocvar{pre}: \coqdocvar{meta} \ensuremath{\rightarrow} \coqdocvar{Any} \ensuremath{\rightarrow} \coqdocvar{Any} \ensuremath{\rightarrow} \coqdocvar{option} \coqdocvar{ord} \ensuremath{\rightarrow} \coqdocvar{rProp};\coqdoceol
\coqdocindent{1.00em}
\coqdocvar{post}: \coqdocvar{meta} \ensuremath{\rightarrow} \coqdocvar{Any} \ensuremath{\rightarrow} \coqdocvar{Any} \ensuremath{\rightarrow} \coqdocvar{rProp};\coqdoceol
\coqdocnoindent
\}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Definition} \coqdocvar{spectable}: \coqdockw{Type} := \coqdocvar{string} \end{coqdoccode}
\hspace{-1pt}$\fpfn{}$\hspace{-5pt} \begin{coqdoccode}
 \coqdocvar{spec};\coqdoceol
\coqdocnoindent
\end{coqdoccode}


==> coq/behavior.tex <==
\begin{coqdoccode}
\coqdocnoindent
\coqdockw{CoInductive} \coqdocvar{beh}: \coqdockw{Type} := \ensuremath{|} \coqdocvar{done} (\coqdocvar{retv}: \coqdocvar{Z}) \ensuremath{|} \coqdocvar{spin} \ensuremath{|} \coqdocvar{ub} \ensuremath{|} \coqdocvar{nb} \ensuremath{|} \coqdocvar{cons} (\coqdocvar{hd}: \coqdocvar{event}) (\coqdocvar{tl}: \coqdocvar{beh}).\coqdoceol
\coqdocemptyline
\coqdocnoindent
\begin{coqdoccomment}
\coqdocindent{0.50em}
add\coqdocindent{0.50em}
behavioral\coqdocindent{0.50em}
refinement\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\end{coqdoccode}


==> coq/ems.tex <==
\begin{coqdoccode}
\coqdocnoindent
\coqdockw{Variant} \coqdocvar{primE}: \coqdockw{Type} \ensuremath{\rightarrow} \coqdockw{Type} :=\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Choose} (\coqdocvar{X}: \coqdockw{Type}): \coqdocvar{primE} \coqdocvar{X}\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Take} (\coqdocvar{X}: \coqdockw{Type}): \coqdocvar{primE} \coqdocvar{X}\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Syscall} (\coqdocvar{fn}: \coqdocvar{string}) (\coqdocvar{args}: \coqdocvar{list} \coqdocvar{Z}): \coqdocvar{primE} \coqdocvar{Z}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Variant} \coqdocvar{modE}: \coqdockw{Type} \ensuremath{\rightarrow} \coqdockw{Type} :=\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Call} (\coqdocvar{fn}: \coqdocvar{string}) (\coqdocvar{args}: \coqdocvar{Any}): \coqdocvar{modE} \coqdocvar{Any}\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Put} (\coqdocvar{st}: \coqdocvar{Any}): \coqdocvar{modE} \coqdocvar{unit}\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Get}: \coqdocvar{modE} \coqdocvar{Any}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Definition} \coqdocvar{emsE}: \coqdockw{Type} \ensuremath{\rightarrow} \coqdockw{Type} := \coqdocvar{primE} +' \coqdocvar{modE}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Definition} \coqdocvar{function} \coqdocvar{E}: \coqdockw{Type} := \coqdocvar{Any} \ensuremath{\rightarrow} \coqdocvar{itree} \coqdocvar{E} \coqdocvar{Any}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Record} \coqdocvar{ems}: \coqdockw{Type} := \coqdocvar{mk\_ems} \{ \begin{coqdoccomment}
\ems{}\end{coqdoccomment}
\coqdoceol
\coqdocindent{1.00em}
\coqdocvar{mn}: \coqdocvar{string};\coqdoceol
\coqdocindent{1.00em}
\coqdocvar{functions}: \coqdocvar{string} \end{coqdoccode}
\hspace{-1pt}$\fpfn{}$\hspace{-5pt} \begin{coqdoccode}
 \coqdocvar{function} \coqdocvar{emsE};\coqdoceol
\coqdocindent{1.00em}
\coqdocvar{initial\_st}: \coqdocvar{Any};\coqdoceol
\coqdocnoindent
\}.\coqdoceol
\end{coqdoccode}


==> coq/imp.tex <==
\begin{coqdoccode}
\coqdocnoindent
\coqdockw{Inductive} \coqdocvar{expr} : \coqdockw{Type} := ... \begin{coqdoccomment}
omitted\end{coqdoccomment}
\coqdoceol
\coqdocemptyline
\coqdocnoindent
\begin{coqdoccomment}
\coqdocindent{0.50em}
use\coqdocindent{0.50em}
BNF\coqdocindent{0.50em}
notation\coqdocindent{0.50em}
and\coqdocindent{0.50em}
present\coqdocindent{0.50em}
only\coqdocindent{0.50em}
selected\coqdocindent{0.50em}
things\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\coqdockw{Inductive} \coqdocvar{stmt} : \coqdockw{Type} :=\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Skip}                           \begin{coqdoccomment}
;\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Assign} (\coqdocvar{x}: \coqdocvar{string}) (\coqdocvar{e}: \coqdocvar{expr})    \begin{coqdoccomment}
x\coqdocindent{0.50em}
=\coqdocindent{0.50em}
e\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Seq}    (\coqdocvar{a} \coqdocvar{b}: \coqdocvar{stmt})            \begin{coqdoccomment}
a\coqdocindent{0.50em}
;\coqdocindent{0.50em}
b\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{If}     (\coqdocvar{i}: \coqdocvar{expr}) (\coqdocvar{t} \coqdocvar{e}: \coqdocvar{stmt}) \begin{coqdoccomment}
if\coqdocindent{0.50em}
(i)\coqdocindent{0.50em}
then\coqdocindent{0.50em}
\{\coqdocindent{0.50em}
t\coqdocindent{0.50em}
\}\coqdocindent{0.50em}
else\coqdocindent{0.50em}
\{\coqdocindent{0.50em}
e\coqdocindent{0.50em}
\}\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{CallFun} (\coqdocvar{x}: \coqdocvar{string}) (\coqdocvar{f}: \coqdocvar{gname}) (\coqdocvar{args}: \coqdocvar{list} \coqdocvar{expr}) \begin{coqdoccomment}
\coqdocindent{0.50em}
x\coqdocindent{0.50em}
=\coqdocindent{0.50em}
f(args),\coqdocindent{0.50em}
by\coqdocindent{0.50em}
name\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{CallPtr} (\coqdocvar{x}: \coqdocvar{string}) (\coqdocvar{p}: \coqdocvar{expr}) (\coqdocvar{args}: \coqdocvar{list} \coqdocvar{expr})  \begin{coqdoccomment}
\coqdocindent{0.50em}
x\coqdocindent{0.50em}
=\coqdocindent{0.50em}
f(args),\coqdocindent{0.50em}
by\coqdocindent{0.50em}
pointer\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{CallSys} (\coqdocvar{x} : \coqdocvar{var}) (\coqdocvar{f} : \coqdocvar{gname}) (\coqdocvar{args} : \coqdocvar{list} \coqdocvar{expr}) \begin{coqdoccomment}
\coqdocindent{0.50em}
x\coqdocindent{0.50em}
=\coqdocindent{0.50em}
f(args),\coqdocindent{0.50em}
system\coqdocindent{0.50em}
call\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{AddrOf} (\coqdocvar{x}: \coqdocvar{string}) (\coqdocvar{X}: \coqdocvar{gname})         \begin{coqdoccomment}
\coqdocindent{0.50em}
x\coqdocindent{0.50em}
=\coqdocindent{0.50em}
\&X\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Malloc} (\coqdocvar{x}: \coqdocvar{string}) (\coqdocvar{s}: \coqdocvar{expr})          \begin{coqdoccomment}
\coqdocindent{0.50em}
x\coqdocindent{0.50em}
=\coqdocindent{0.50em}
malloc(s)\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Free} (\coqdocvar{p}: \coqdocvar{expr})                      \begin{coqdoccomment}
\coqdocindent{0.50em}
free(p)\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdockw{Load} (\coqdocvar{x}: \coqdocvar{string}) (\coqdocvar{p}: \coqdocvar{expr})            \begin{coqdoccomment}
\coqdocindent{0.50em}
x\coqdocindent{0.50em}
=\coqdocindent{0.50em}
*p\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Store} (\coqdocvar{p}: \coqdocvar{expr}) (\coqdocvar{v}: \coqdocvar{expr})          \begin{coqdoccomment}
\coqdocindent{0.50em}
*p\coqdocindent{0.50em}
=\coqdocindent{0.50em}
v\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
\ensuremath{|} \coqdocvar{Cmp} (\coqdocvar{x}: \coqdocvar{string}) (\coqdocvar{a}: \coqdocvar{expr}) (\coqdocvar{b}: \coqdocvar{expr})  \begin{coqdoccomment}
\coqdocindent{0.50em}
memory\coqdocindent{0.50em}
accessing\coqdocindent{0.50em}
equality\coqdocindent{0.50em}
comparison\coqdocindent{0.50em}
\end{coqdoccomment}
\coqdoceol
\coqdocnoindent
.\coqdoceol
\end{coqdoccode}


==> coq/mod.tex <==
\begin{coqdoccode}
\coqdocnoindent
\coqdockw{Variant} \coqdocvar{symbol}: \coqdockw{Type} := \ensuremath{|} \coqdocvar{Gfun} \ensuremath{|} \coqdocvar{Gvar} (\coqdocvar{data}: \coqdocvar{Z}). \end{coqdoccode}
\begin{coqdoccode}
 \coqdockw{Definition} \coqdocvar{symbols}: \coqdockw{Type} := (\coqdocvar{string} \end{coqdoccode}
\hspace{-1pt}$\fpfn{}$\hspace{-5pt} \begin{coqdoccode}
 \coqdocvar{symbol}).\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Definition} \coqdocvar{emsmod}: \coqdockw{Type} := \coqdocvar{symbols} \ensuremath{\times} (\coqdocvar{symbols} \ensuremath{\rightarrow} \coqdocvar{ems}).\coqdoceol
\coqdocemptyline
\end{coqdoccode}


==> discussion.tex <==
\section{Evaluation}
\label{sec:discussion}

\begin{wraptable}{r}{5.0cm}
\vspace{-5mm}
%% \begin{minipage}{\linewidth}
\centering
%% \parbox{0.33\linewidth}{
\begin{tabu}{l @{\;}|@{\;} l @{\;}|@{\;} l}
Portion & Def & Proof \\
\hline
\ems & 2584 & 3025 \\
SL-specific & 5709 & 3632 \\
\imp-specific & 3770 & 4129 \\ %% imp
Examples & 3082 & 3054 \\ %% examples + mem.
Coq libraries & 2689 & 850 \\ %% extraction && libraries
\hline
Total & 17834 & 14690 \\
\end{tabu}
\label{table:evaluation}
%% }
%% \end{minipage}
\vspace{-3mm}
\end{wraptable}

The right table shows the SLOC of the whole development (counted by \code{coqwc}).
\ems{} and its meta-theory amount to 5609 SLOC, SL-specific theory (including \gen{}, proof
mode, translations, and spec erasure theorem) to 9341 SLOC, \imp{}-specific theory (including
syntax, semantics, its compiler, and compiler verification) to 7899 SLOC, verification
examples (Cannon, Mem, Stack, Echo, Repeat, and Landin's knot) to 6136 SLOC, and general
purpose Coq libraries to 3539 SLOC. In total, our Coq definitions amount to 17834 SLOC and
proofs to 14690 SLOC.

The proof effort for verifying each example in \crems is split into two:
$(i)$ that for reasoning about SL entailment, which would be comparable to that in \iris because we use IPM and prove essentially similar goals,
and
$(ii)$ that for simulation reasoning, which was quite straightforward in all the examples thanks to our tactics.
%% When verifying examples, proof effort for resource reasoning is comparable to that of Iris
%% (since we use IPM), and proof effort for simulation reasoning is also minor thanks to our
%% proof mode.

Vertical compositionality of CR (\ie gradual abstraction) also simplified the proof of meta theory of \crems.
For instance, the spec erasure theorem (\Cref{thm:spec-erasure}) is established by
transitively composing six contextual refinements, two major ones of which are
$(i)$ removing \ASSUME{} and \GUARANTEE{} while concretizing the measure information
and $(ii)$ removing pure calls by proving their termination using the measure information.

%% assume/guarantees and resources while concretizing measure parameter (which was passed implicitly via \kwchoose{} and \kwtake{}),
%% Two major layers in the former are 
%% In the proof of meta-theory of \crems, we also used 
%% We report that we heavily relied on gradual abstraction in our meta-theory, where spec
%% erasure theorem without context (\Cref{thm:erasure-closed}) comprises three layers and the
%% main spec erasure theorem (\Cref{thm:spec-erasure}) comprise three additional layers.

All the examples in the paper are extracted to OCaml programs, and we indeed found bugs by testing before verification.
%% Our examples, embedded in \ems, can be extracted to OCaml and executed.
For extraction, all the events are handled inside Coq except for \EventE{},
which are handled by special handlers written in OCaml.
Specifically, we wrote a few handlers doing IO for $\syscallE$
and a handler for $\chooseE$ and $\takeE$, which asks the user for a nondeterministic choice
(currently only supports \vint{}).
For testing, we extracted both implementations and abstractions, executed them and compared the results.
Interestingly, we found two mis-downcast bugs in the abstraction of \Echo{} by testing before verification.
Also we can extract and run even the abspecs although it would introduce so much nondeterminism.

%% It also runs at abspec level but there are too much non-determinism.

%% At the moment, we use very simple one supporting \eg standard IO (for
%% \syscallE) and choosing an integer value (for \chooseE), which is sufficient for our
%% examples.
%% Notably, the echo example runs well at top level ($|A|$) and \imp level ($I$) via extraction.
%% It also runs at abspec level but there are too much non-determinism.
%% and also assembly level via compilation.
%% With these, we did differential testing before verification and discovered some bugs.

%% will share our experience, current limitations, and possible future works.
%% \yj{say that execution is useful. segfault type error}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> figures/definitions.tex <==
\section{Definitions}

\begin{figure}[t]
\begin{minipage}{0.5\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]

\EventE : $\equiv$
| \chooseE: $\forall$ X, \unitset $\effectarrow$ X
| \takeE: $\forall$ X, \unitset $\effectarrow$ X
| \syscallE: \fname $\times$ \anyv $\effectarrow$ \anyv

\EmsE : $\equiv$
| \EventE
| \putE: \anyv $\effectarrow$ \unitset
| \getE : \unitset $\effectarrow$ \anyv
| \callE : \fname $\times$ \anyv $\effectarrow$ \anyv

\mfun E $\equiv$ (\mname $\times$ \anyv) $\rightarrow$ \itree{E}{\anyv}

\ems $\equiv$ \{
  name: string;
  functions: \fname $\fpfn$ \mfun{\EmsE};
  initial_state: \anyv;
\}

\SpcE $\equiv$
| \EmsE
| \ApcE : \unitset $\effectarrow$ \unitset

\ord $\equiv$
| ord_top
| ord_pure (o: ordinal)

\rprop $\equiv$ $\monoid$ $\rightarrow$ $\propb$

\SLspec $\equiv$ (X: Set, X $\rightarrow$ (\anyv $\rightarrow$ (\anyv $\times$ \ord) $\rightarrow$ \rprop)
                        $\times$ (\anyv $\rightarrow$ \anyv $\rightarrow$ \rprop))

\SLspecs $\equiv$ \fname $\fpfn$ \SLspec

\spc $\equiv$ \{
  name: string;
  functions$_{\text{friend}}$: \fname $\fpfn$ \mfun{\SpcE};
  functions$_{\text{context}}$: \fname $\fpfn$ \mfun{\SpcE};
  specs: \SLspecs;
  initial\_state: \anyv;
  initial\_resource: \monoid;
\}

$\spcfun{S_{context}}{(f:\text{\mfun \SpcE})}{(S:\text{\SLspec})}{(g:\text{\mfun \SpcE})}$ : \mfun \EmsE

$\spcmod{(S_{context}:\text{\SLspecs})}{(A:\text{\spc})}{(S:\text{\SLspecs})}$ $\equiv$ \{
  name: A.name;
  functions: $\lambda$f.$\spcfun{S_{context}}{\text{functions}_{\text{friend}}(\text{f})}{\text{specs}(\text{f})}{\text{functions}_{\text{context}}(\text{f})}$
  initial\_state: (A.initial\_state, $\upcast(\text{A.initial\_resource})$);
\}

\end{Verbatim}
\end{minipage}
\end{figure}



\begin{figure}[t]
\begin{minipage}{0.5\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
\SLcall ($S_{context}$: \SLspecs) (fn: \fname, arg$_\text{logical}$: \anyv) $\equiv$
  (X, spec) := $S_{context}$(fn);
  x := \chooseE(X);
  (P, Q) := spec(x);
  arg$_\text{physical}$ := \chooseE(\anyv);
  ord_next := \chooseE(\ord);
  \kwguarantee(ord\_next < ord\_cur);
  (argr, fr, mr_new) := \chooseE($\monoid$ $\times$ $\monoid$ $\times$ $\monoid$);
  \kwguarantee($\mvalFull$(argr * fr * ctx * mr\_new));
  (_, st) := \getE;
  \putE((mr\_new, st));
  \kwguarantee(P arg$_\text{logical}$ arg$_\text{physical}$ ord\_next argr);
  ret$_\text{physical}$ := fn(arg$_\text{physical}$);
  ret$_\text{logical}$ := \takeE(\anyv);
  (mr, _) := \getE;
  (retr, ctx) := \takeE($\monoid$ $\times$ $\monoid$);
  \kwassume($\mvalFull$(retr * fr * ctx * mr));
  \kwassume(Q ret$_\text{logical}$ ret$_\text{physical}$ retr);
  ret$_\text{logical}$

\SLpre (P: \anyv $\rightarrow$ \anyv $\rightarrow$ \ord $\rightarrow$ $\monoid$ $\rightarrow$ $\propb$) (arg$_\text{physical}$: \anyv) $\equiv$
  arg$_\text{logical}$ := \takeE(\anyv);
  \kwvar ord\_cur := \takeE(\ord);
  (argr, ctx) := \takeE($\monoid$ $\times$ $\monoid$);
  (mr, _) := \getE;
  \kwassume($\mvalFull$(argr * ctx * mr));
  \kwassume(P arg$_\text{physical}$ (arg$_\text{logical}$, ord\_cur) argr);
  arg$_\text{logical}$

\SLpost (Q: \anyv $\rightarrow$ \anyv $\rightarrow$ $\monoid$ $\rightarrow$ $\propb$) (ret$_\text{logical}$: \anyv) $\equiv$
  ret$_\text{physical}$ := \chooseE(\anyv);
  (retr, mr\_new) := \chooseE($\monoid$ $\times$ $\monoid$);
  \kwguarantee($\mvalFull$(retr * ctx * mr\_new));
  (_, st) := \getE;
  \putE((mr_new, st));
  \kwguarantee(Q ret$_\text{physical}$ ret$_\text{logical}$ retr);
  ret$_\text{physical}$

\SLIPC ($S_{context}$: \SLspecs) $\equiv$
  \kwvar o := \chooseE(ordinal);
  \kwwhile(\chooseE(bool))
    (fn, arg) := \chooseE(\fname $\times$ \anyv);
    \SLcall($S_{context}$)(fn)(arg);
    o\_new := \chooseE(ordinal);
    \kwguarantee(o\_new < o);
    o := o\_new

\SLbody($S_{context}$)(body) $\equiv$ body[\callE $\mapsto$ \SLcall($S_{context}$),
                               \ApcE $\mapsto$ \SLIPC($S_{context}$)]

\end{Verbatim}
\end{minipage}
\end{figure}

\begin{figure}[t]
\begin{minipage}{0.5\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]

$\spcfun{S_{context}}{(f:\text{\mfun \SpcE})}{(S:\text{\SLspec})}{(g:\text{\mfun \SpcE})}$ : $\equiv$
  \kwfun (mn: \mname, arg: \anyv) =>
    friend := \takeE(bool);
    \kwif(friend)
      (X, spec) := $S$;
      x := \takeE(X);
      (P, Q) := spec(x);
      arg := \SLpre(P)(arg);
      ret := \SLbody($S_{context}$)(f(mn,arg));
      \SLpost(Q)(ret)
    \kwelse
      g(mn, arg)

\end{Verbatim}
\end{minipage}
\end{figure}

\begin{figure}[t]
\begin{minipage}{0.5\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]

\spcmodforget{(A:\text{\spc})}{friends} $\equiv$ \{
  name: A.name;
  functions: $\lambda$f.\spcfunforget{functions$_{\text{friend}}$(f)}{functions$_{\text{context}}$(f)}{friends};
  initial\_state: A.initial\_state;
\}

\spcfunforget{f: \mfun \SpcE}{g: \mfun \SpcE}{friends} $\equiv$
  \kwfun (mn: \mname, arg: \anyv) =>
    \kwif(mn $\in$ friends)
      f(mn, args)[\ApcE $\mapsto$ \kwskip]
    \kwelse
      g(mn, args)[\ApcE $\mapsto$ \kwskip]

\end{Verbatim}
\end{minipage}
\end{figure}


==> figures/echo.tex <==
\begin{figure}[t]
$I_\Echo$ := \hfill\mbox{}\\
\begin{minipage}[t]{0.33\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Echo]
\kwdef echo([]\unwrapU{}) $\equiv$
  \kwvar stk := Stack.new();
  Echo.input(stk);
  Echo.output(stk)
\end{Verbatim}
\end{minipage}%
\begin{minipage}[t]{0.36\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
\kwdef input([stk: \vval{}]\unwrapU{}) $\equiv$
  \kwvar v := IO.getint();
  \kwif (v == \exitval) \kwthen 0
  \kwelse \{ Stack.push(stk, v);
         Echo.input(stk) \}
\end{Verbatim}
\end{minipage}%
\begin{minipage}[t]{0.31\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
\kwdef output([stk: \vval{}]\unwrapU{}) $\equiv$
  \kwvar v := Stack.pop(stk);
  \kwif (v == \exitval) \kwthen 0
  \kwelse \{ IO.putint(v);
         Echo.output(stk) \}
\end{Verbatim}
\end{minipage}
\\[1mm]
$A_\Echo$ := \hfill\mbox{}\\[1mm]
\begin{minipage}{0.265\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Echo]
\kwdef echo = 
 \kwfriend,\kwcontext([]\unwrapU{}) $\equiv$
  \kwvar stk:\unwrapN{} list \vint
    := Echo.input([]);
  Echo.output(stk)
\end{Verbatim}
\end{minipage}%
\begin{minipage}{0.355\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
\kwdef input =
 \kwfriend(stk:\unwrapN{} list \vint) $\equiv$
  \kwvar v:\unwrapU{} \vint := $\code{IO.getint()}$;
  \kwif (v == \exitval) \kwthen stk
  \kwelse Echo.input(v::stk)
 \kwcontext(\_) $\equiv$ \kwub
\end{Verbatim}
\end{minipage}%
\begin{minipage}{0.3\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
\kwdef output =
 \kwfriend(stk:\unwrapN{} list \vint) $\equiv$
  \kwmatch stk \kwwith | [] => ()
  | hd::tl => IO.putint(hd);
              Echo.output(tl) \kwend
 \kwcontext(\_) $\equiv$ \kwub
\end{Verbatim}
\end{minipage}%
\hfill\mbox{}
\\[2mm]
$\mires_\Echo$ := $\munit$\hfill\mbox{}
\\
\begin{minipage}[t]{\textwidth}
\small$\begin{array}{@{}l@{}l@{\,}l@{\;}l@{}}
S_\Echo := \{
&
\code{Echo.echo}{:}
&
\snone,
&
\\&
\code{Echo.input}{:}
&
\forall \handle\!:\!\vptr.
&
\curlybracket{\lambda\,\argp\,\argv\,\argo.\; \exists \lst:\vlist\;\vint.\; \rplift{\argo = \otop \lland \argp = \upcast{[\handle]} \lland \argv = \upcast{\lst}} * \isestack{\handle}{\lst}}
\\&
&&
\curlybracket{\lambda\,\retp\,\retv.\;\exists \lst:\vlist\;\vint.\; \rplift{\retp \in \upcast{\vval} \lland \retv = \upcast{\lst}} * \isestack{\handle}{\lst}},
\\&
\code{Echo.output}{:}
&
\forall \handle\!:\!\vptr.
&
\curlybracket{\lambda\,\argp\,\argv\,\argo.\; \exists \lst:\vlist\;\vint.\; \rplift{\argo = \otop \lland \argp = \upcast{[\handle]} \lland \argv = \upcast{\lst}} * \isestack{\handle}{\lst}}
\\&
&&
\curlybracket{\lambda\,\retp\,\retv.\;\exists \lst:\vlist\;\vint.\; \rplift{\retp \in \upcast{\vval} \lland \retv = \upcast{\lst}} * \isestack{\handle}{\lst}}
\hfill\}
\end{array}$
\end{minipage}
\\
where $\isestack{\handle}{\lst} = \rplift{\lstnz(\lst)} * \isstack{\handle}{\lst}$
\hfill\mbox{}
\myhrule
\caption{An implementation and its abspec for the module \Echo{}.}
\label{fig:echo}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/embedding.tex <==
\begin{figure}[t]
\hfill
\begin{minipage}{0.525\textwidth}

{
\small
$\toabs{A}{N} \defeq$ $( A.\code{name},\; A.\code{init},\;$ $\lambda \fn.\; \code{\transA} (N, A.\code{funs} \; \fn) )$ \\
}%

\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\small]
\trm{\transA}$(N, (frd, ctx))$: \trm{fundef}(\EmsE) $\defeq{}\lambda{}\argp.$
  \kwvar mn := \kwgetcaller{}();
  \kwif(mn $\in$ $N$) $frd$($\argp$)[IPC $\mapsto$ \kwskip]
  \kwelse   \hspace{0.13cm}    $ctx$($\argp$)[IPC $\mapsto$ \kwskip]

\end{Verbatim}

{
\small
$\spcmod{S}{A, \mires}{S_{a}} \defeq$ $( A.\code{name},\; (A.\code{init}, \upcast{\mires}),\;$\\
\-\hspace{1.32cm}  $\lambda\, \fn.\; \code{\transAS}(S,\;A.\code{funs} \; \fn, \; S_{a}\;\fn) )$ \\
}%

\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\small]
\trm{\transAS}$(S, (frd, ctx), s)$: \trm{fundef}(\EmsE) $\defeq{}\lambda{}\argp.$
  \kwvar is\_friend := \kwtake(bool);
  \kwif(is\_friend) $\textrm{\AS{}Fun}(S, s, frd)(x)$
  \kwelse          $\textrm{\AS{}Fun}(S, \snone,\,ctx)(x)$

\end{Verbatim}

\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\small]
\trm{\AS{}Fun}($S$, $s$, fun: \trm{fundef}(\SpcE)) $\defeq$ $\lambda{}\argp.$
  \kwvar ($\Meta$, PQ) := $s$;
  \kwvar \meta{} := \kwtake(\Meta);
  \kwvar (P, Q) := PQ(\meta{});
  \kwvar ($\argv$, $\argo$, \eres{}) := \AS{}Pre(P,$\argp$);
  \kwmatch $\argo$ \kwwith
  | None => \kwvar ($\retv$, \eres{}) :=
    \AS{}Body($S$, $\argo$, \eres{}, fun($\argv$));
  | Some o =>
    \kwvar (\_, \eres{}) := \AS{}IPC($S$, $\argo$, \eres{});
    \kwvar $\retv$ := \kwchoose(\tyany);
  \kwend;
  \AS{}Post(Q)($\retv$, \eres{})

\end{Verbatim}

\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\small]
\AS{}Body($S$, $\argo$, \eres{}, body) $\defeq$ body[
 \callE fn $\argv$ $\mapsto$ $\lambda{}\eres{}.$ \trm{\AS{}Call}($S$,$\argo$,\eres{},fn,$\argv$),
   \hspace{0.59cm} \ApcE $\mapsto$ $\lambda{}\eres{}.$ \trm{\AS{}IPC}($S$,$\argo$,\eres{})]
\end{Verbatim}

\end{minipage}%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{0.470\textwidth}

\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\small]
\trm{\AS{}Call}($S$, $\argo$, \eres{}, fn, $\argv$) $\defeq$
  \kwvar ($\Meta$, PQ) := $S$(fn);
  \kwvar \meta := \kwchoose($\Meta$);
  \kwvar (P, Q) := PQ(\meta);
  \kwvar ($\argp$, $\argo$') := \kwchoose(\anyv $\times$ \ord);
  \kwguarantee($\argo$' $\sqsubset \argo$);
  \kwvar (\kwap, \lres, $\mres_{0}$) := \kwchoose(\_);
  \kwguarantee$(\mval(\kwap+\lres+\mres_{0}+\eres{}))$;
  \kwvar (\_, st) := \kw{get};
  \kw{put}(($\mres_{0}$, st));
  \kwguarantee(P $\argv$ $\argp$ $\argo$' \kwap);
  \kwvar $\retp$ := \kwcall fn $\argp$;
  \kwvar $\retv$ := \kwtake(\anyv);
  \kwvar ($\mres_{1}$, \_) := \kw{get};
  \kwvar \kwrp := \kwtake($\monoid$);
  \kwvar \eres{} := \kwtake($\monoid$);
  \kwassume$(\mval(\kwrp+\lres+\mres_{1}+\eres{}))$;
  \kwassume(Q $\retv$ $\retp$ \kwrp);
  ($\retv$, \eres{})

\trm{\AS{}IPC}($S$, $\argo$, \eres{}) $\defeq$
  \kwvar i := \kwchoose(\ordinal);
  \kwwhile(\kwchoose(bool))
    \kwvar (fn, $\argv$) := \kwchoose(\fname $\times$ \anyv);
    (\_, \eres{}) := \trm{\AS{}Call}($S$,$\argo$,\eres{},fn,$\argv$);
    i := \kwchoose(\{i' $\in$ \ordinal | i' < i\})
  ((), \eres{})
\end{Verbatim}
\end{minipage}
%% \kwvar (\kwrp, \eres{}) := \kwtake($\monoid\times\monoid$);
%% \SLIPC ($S_{\all}$: \trm{specs}) $\equiv$
%%   \kwvar o$_{0}$ := \chooseE(ordinal);
%%   \kwwhile(\chooseE(bool))
%%     \kwvar (fn, arg) := \chooseE(\fname $\times$ \anyv);
%%     \SLcall($S_{\all}$)(fn, arg);
%%     \kwvar o$_{1}$ := \chooseE(ordinal);
%%     \kwguarantee(o$_{1}$ < o$_{0}$);
%%     o$_{0}$ := o$_{1}$
\myhrule
\caption{Translations of pre-abstraction into abspec and abstraction (\code{\AS{}Pre} and \code{\AS{}Post} are omitted).}
\label{formal:embedding}
\end{figure}


==> figures/hoare-logic.tex <==
\begin{figure}[t]
$I_\code{Main}$ :=
\begin{minipage}[t]{0.4\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Main]
\kwdef main() $\equiv$
  \kwvar x := 40;
  \kwvar r := F.f(x);
  \kwif (r\%2 == 1) \kwthen \prt(42) \kwelse 1/0
\end{Verbatim}
\end{minipage}%
\hfill%
$I_\code{F}$ :=
\begin{minipage}[t]{0.39\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule F]
\kwdef f(x) $\equiv$
  \kwvar r := x*x/4 + x + 1;
  \prt(r);
  r
\end{Verbatim}
\end{minipage}%
\\[1mm]
\begin{minipage}[t]{0.51\textwidth}
$S_\code{Main}$ := $\setofz{ \hoare{\TRUE} {\code{Main.main}} {\TRUE} }$
\end{minipage}%
\hfill%
\begin{minipage}[t]{0.44\textwidth}
$S_\code{F}$ := $\setofz{ \hoare{\lambda x.\; x \modcode 4 = 0} {\code{F.f}} {\lambda \valr.\; \valr \modcode 4 = 1} }$
\end{minipage}%
\\[1mm]
$A_\Main$ :=
\begin{minipage}[t]{0.4\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Main]
\kwdef main() $\equiv$
  \kwvar x := 40;
  \kwvar r := F.f(x);
  \fbox{\prt(42)}
\end{Verbatim}
\end{minipage}%
\hfill%
$A_\code{F}$ :=
\begin{minipage}[t]{0.38\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule F]
\kwdef f(x) $\equiv$
  \kwvar r := \fbox{(x/2 + 1)**2};
  \prt(r);
  r
\end{Verbatim}
\end{minipage}%
\\[1mm]
\begin{minipage}[t]{0.5\textwidth}
$\spcmod{S_\code{Main} \cup S_\code{F}}{A_\code{Main}}{S_\code{Main}}$ :=\\
\hspace*{10pt}\begin{minipage}[t]{0.4\textwidth}  
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Main]
\kwdef main() $\equiv$
  \kwvar x := 40;
 \mydashbox{blue}{10pc}{\kwguarantee(x\%4 == 0);}
  \kwvar r := F.f(x);
 \mydashbox{red}{10pc}{\kwassume(r\%4 == 1);}
  \prt(42)
\end{Verbatim}
\end{minipage}%
\end{minipage}%
\hfill%  
\begin{minipage}[t]{0.445\textwidth}
$\spcmod{S_\code{Main} \cup S_\code{F}}{A_\code{F}}{S_\code{F}}$ :=\\
\hspace*{10pt}\begin{minipage}[t]{0.4\textwidth}  
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule F]
\kwdef f(x: int) $\equiv$
 \mydashbox{red}{10pc}{\kwassume(x\%4 == 0);}
  \kwvar r := (x/2 + 1)**2;
  \prt(r);
 \mydashbox{blue}{10pc}{\kwguarantee(r\%4 == 1);}
  r
\end{Verbatim}
\end{minipage}%
\end{minipage}%
\myhrule
\caption{Implementations, HL specifications, Abstractions, and Abspecs for \Main{} and \MF{}}
\label{fig:hoare-logic}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/pcm.tex <==
\begin{figure}[t]
\small
\[
  \textrm{PCM is a quadruple } (\monoid,\; \madd,\; \wdef,\; \munit) \in (Set \times (\monoid
  \rightarrow \monoid \rightarrow  \monoid) \times \mathcal{P}(\monoid) \times \monoid) \;
  \textrm{satisfying:}
\]
\[
\begin{array}{r@{\;}l@{\hspace{2.3cm}}l}
    \forall a, b, c, & a \madd (b \madd c) = (a \madd b) \madd c                  & \caselabel{PCM-ASSOC}\;     \\
    \forall a, b,    & a \madd b = b \madd a                              & \caselabel{PCM-COMM}\;      \\
    \forall a,       & \munit \madd a = a                             & \caselabel{PCM-UNIT}\;      \\
                     & \wdef(\munit)                          & \caselabel{PCM-UNIT-VALID}\; \\
    \forall a, b,    & \wdef (a \madd b) \Rightarrow \wdef(a) & \caselabel{PCM-MON}\; \\
\end{array}
\]
\\
\vspace{3mm}
\[x \rightsquigarrow x' \defeq \forall ctx,\; \wdef (ctx \madd x) \Rightarrow
  \wdef (ctx \madd x')
\]
%% \\
%% \vspace{7mm}

\caption{Partial Commutative Monoids}
\label{fig:formal:pcm}
\end{figure}


==> figures/sep-logic.tex <==
\begin{figure}[t]
$I_\Main$ :=
\begin{minipage}[t]{0.31\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Main]
\kwdef main() $\equiv$
  \kwrepeat \numfire \{
    \kwvar r := \Cannon.\fire{}();
    \prt(r)
  \}
\end{Verbatim}
\end{minipage}%
\hfill%
$I_\Cannon$ :=
\begin{minipage}[t]{0.39\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule \Cannon{}]
\kwlocal \powder = 1
\kwdef \fire{}() $\equiv$
  \kwvar r := 1/\powder;
  \prt(r);
  \powder := \powder - 1;
  r
\end{Verbatim}
\end{minipage}%
\\[1mm]
\begin{minipage}[t]{0.41\textwidth}
$S_\Main$ :=
$\left\{
\begin{array}{@{}r@{}l@{}l@{}}
\hoare{\slball}{\code{Main.main}} {\TRUE}
\end{array}
\right\}$
\end{minipage}%
\hfill%
\begin{minipage}[t]{0.495\textwidth}
$S_\Cannon$ :=
$\left\{
\begin{array}{@{}r@{}l@{}l@{}}
\hoare{\slball} {\code{\Cannon.\fire}} {\Ret\valr. \valr = 1}
\end{array}
\right\}$
\end{minipage}%
\\[1mm]
\begin{minipage}[t]{0.4\textwidth}
$\mires_\Main$ := $\kwemp$
\end{minipage}%
\hfill%
\begin{minipage}[t]{0.495\textwidth}
$\mires_\Cannon$ := $\ready$
\end{minipage}%
\\[1mm]
$A_\Main$ :=
\begin{minipage}[t]{0.31\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Main]
\kwdef main() $\equiv$
  \kwrepeat \numfire \{
    \kwvar r := \Cannon.\fire{}();
    \prt(\fbox{1})
  \}
\end{Verbatim}
\end{minipage}%
\hfill%
$A_\Cannon$ :=
\begin{minipage}[t]{0.39\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule \Cannon{}]
\fbox{\phantom{local n = 1}}
\kwdef \fire{}() $\equiv$
  \kwvar r := \fbox{1};
  \prt(\fbox{1});
  \fbox{\phantom{n := n - 1;}}
  r
\end{Verbatim}
\end{minipage}%
\\[1mm]
\begin{minipage}[t]{0.5\textwidth}
$\spcmod{S_\Main \cup S_\Cannon}{(A_\Main,\mires_\Main)}{S_\Main}$ :=\\
\hspace*{10pt}\begin{minipage}[t]{0.4\textwidth}  
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Main]
\boilerplate{\kwlocal \mres :=} \hl{$\kwemp$}
\kwdef main() $\equiv$
  \boilerplate{\kwvar \lres := \kwemp;}
 \mydashbox{red}{14pc}{\ASSUME($\lambda$\res. \res == \ball)}
  \kwrepeat \numfire \{
   \mydashbox{blue}{13.25pc}{\GUARANTEE($\lambda$\res. \res == \ball)}
    \kwvar r := \Cannon.\fire{}();
   \mydashbox{red}{13.25pc}{\ASSUME($\lambda$\res. \res == \kwemp && r == 1)}
    \prt(1)
  \}
 \mydashbox{blue}{14pc}{\GUARANTEE($\lambda$\res. \res == \kwemp)}
\end{Verbatim}
\end{minipage}%
\end{minipage}%
\hfill%
\begin{minipage}[t]{0.5\textwidth}
$\spcmod{S_\Main \cup S_\Cannon}{(A_\Cannon,\mires_\Cannon)}{S_\Cannon}$ :=\\
\hspace*{10pt}\begin{minipage}[t]{0.4\textwidth}  
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule \Cannon{}]
\boilerplate{\kwlocal \mres :=} \hl{$\ready$}
\kwdef \fire{}() $\equiv$
  \boilerplate{\kwvar \lres := \kwemp;}
 \mydashbox{red}{14pc}{\ASSUME($\lambda$\res. \res == \ball)}
  \kwvar r := 1;
  \prt(1);
 \mydashbox{blue}{14pc}{\GUARANTEE($\lambda$\res. \res == \kwemp && r == 1)}
  r
\end{Verbatim}
\end{minipage}%
\end{minipage}%
\\[2mm]
\begin{minipage}[t]{0.5\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
\color{red}\ASSUME(Cond) $\equiv$ \{
\color{red}  \kwvar \res := \kwtake(\kwcanonpcm);
\color{red}  \kwassume(Cond(\res));
\color{red}  \lres := \lres + \res;
\color{red}  \kwassume(\mres + \lres != \kwundef);
\color{red}\}
\end{Verbatim}
\end{minipage}%
\hfill%
\begin{minipage}[t]{0.5\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
\color{blue}\GUARANTEE(Cond) $\equiv$ \{
\color{blue}  (\mres, \lres) := \kwfpu(\mres, \lres);
\color{blue}  \kwvar \res := \kwchoose(\kwcanonpcm);
\color{blue}  \kwguarantee(Cond(\res));
\color{blue}  \lres := \kwminus(\lres, \res);
\color{blue}\}
\end{Verbatim}
\end{minipage}%
\myhrule
\caption{Implementations, SL specifications, Initial resources, Abstractions,
  and Abspecs for \Main{} and \Cannon{}}
\label{fig:sep-logic}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/stack1.tex <==
\begin{figure}[t]
$I_\Stack$ :=
\begin{minipage}[t]{0.33\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Stack]
\kwdef new([]\unwrapU{}) $\equiv$
  \kwvar stk := Mem.alloc(1);
  Mem.store(stk, NULL);
  stk
\kwdef push([stk: \vval{}, v: \vval{}]\unwrapU{}) $\equiv$
  \kwvar node := Mem.alloc(2);
  \kwvar hd := Mem.load(stk);
  Mem.store(node, v);
  Mem.store(node+8, hd);
  Mem.store(stk,node)
\kwdef pop([stk: \vval{}]\unwrapU{}) $\equiv$
  \kwvar hd := Mem.load(stk);
  \kwif hd == NULL \kwthen 0
  \kwelse
    \kwvar v := Mem.load(hd);
    \kwvar next := Mem.load(hd+8);
    Mem.store(stk, next);
    Mem.free(hd); Mem.free(hd+8);
    v
\end{Verbatim}
\end{minipage}%
\hfill%
$A^1_\Stack$ :=
\begin{minipage}[t]{0.47\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Stack]
\kwlocal pool := ($\lambda$_. \none)
  : \vptr {$\rightarrow$} \option (\vlist \vval{})
\kwdef new =
 \kwfriend,\kwcontext([]\unwrapU{}) $\equiv$
  \kwvar handle := \kwchoose(\vptr{});
  \kwguarantee(pool handle == \none);
  pool := pool[handle := \some []];
  handle
\kwdef push =
 \kwfriend,\kwcontext([handle: \vptr{}, v: \vval{}]\unwrapU{}) $\equiv$  
  \kwvar stk := unopt\unwrapU{}(pool handle);
  pool := pool[handle := \some (x::stk)]
\kwdef pop =
 \kwfriend,\kwcontext([handle: \vptr{}]\unwrapU{}) $\equiv$
  \kwvar stk := unopt\unwrapU{}(pool handle);
  \kwmatch stk \kwwith | [] => 0
  | v :: stk' =>
    pool := pool[handle := \some stk'];
    v  \kwend
\end{Verbatim}
\end{minipage}
\\[2mm]
$S^1_\Stack$ := $\setofz{\  \code{\Stack.new}:\snone,\  \code{\Stack.push}:\snone,\ \code{\Stack.pop}:\snone\ }$
\hspace*{5pc}$\mires^1_\Stack$ := $\munit$\hfill\mbox{}\\[1mm]
where $\snone = \forall \_:\vunit.\;\hoare{\lambda\,\argp\,\argv\,\argo.\; \rplift{\argo = \otop \lland \argp = \argv}}{}{\lambda\,\retp\,\retv.\; \rplift{\retp = \retv}}$\hfill\mbox{}
\myhrule
\caption{An implementation and its first abspec for the module \Stack{}.}
\label{fig:stack1}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/stack2.tex <==
\begin{figure}[t]
$A^2_\Stack$ := 
\begin{minipage}[t]{0.37\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Stack]
\kwlocal pool := ($\lambda$_. \none)
  : \vptr {$\rightarrow$} \option (\vlist \vval)
\end{Verbatim}
\end{minipage}%
\begin{minipage}[t]{0.27\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
\kwdef new =
 \kwfriend(\_) $\equiv$ \kwnb
 \kwcontext([]\unwrapU{}) $\equiv$ ...
\end{Verbatim}
\end{minipage}%
\begin{minipage}[t]{0.1\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
...


\end{Verbatim}
\end{minipage}%
\hfill\mbox{}
\\[1mm]
$\mires^\twoA_\Stack$ := $\authfull\munit \in \authm{\,(\vptr \rightarrow \exm{\,(\code{\vlist \vval})})} \subseteq \Sigma$\hfill\mbox{}
\\[1mm]
\begin{minipage}[t]{\textwidth}
\small$\begin{array}{@{}l@{}l@{\;}l@{\;}l@{}}
S^\twoA_\Stack := \{
&    
\code{Stack.new}{:}
&    
\forall \_:\vunit.
&
\curlybracket{\lambda\,\argp\,\_\,\argo.\; \rplift{\argo = \opure\;\_ \lland \argp = \upcast{[]}}}
\\&
&&
\curlybracket{\lambda\,\retp\,\_.\; \exists \handle:\vptr.\; \rplift{\retp = \upcast{\handle}} * \isstack{\handle}{[]}},
\\&
\code{Stack.push}{:}
&
\forall (\handle,v,\lst):\vptr \!\times\! \vval \!\times\! \vlist\;\vval.
&
\curlybracket{\lambda\,\argp\,\_\,\argo.\; \rplift{\argo = \opure\;\_ \lland \argp = \upcast{[\handle, v]}} * \isstack{\handle}{\lst}}
\\&
&&
\curlybracket{\lambda\,\retp\,\_.\; \rplift{\retp \in \upcast{\vval}} * \isstack{\handle}{(v :: \lst)}},
\\&
\code{Stack.pop}{:}
&
\forall (\handle,\lst):\vptr \times \vlist\;\vval.
&
\curlybracket{\lambda\,\argp\,\_\,\argo.\; \rplift{\argo = \opure\;\_ \lland \argp = \upcast{[\handle]}} * \isstack{\handle}{\lst}}
\\&
&&
\curlybracket{\lambda\,\retp\,\_.\; \rplift{ \retp = \upcast{\lsthead(\lst,0)}} * \isstack{\handle}{\lsttail(\lst)}}
\hfill\}
\end{array}$
\end{minipage}
\\[1mm]
$\mires^\twoB_\Stack$ := $\authfull\munit \in \authm{\,(\vptr \rightarrow \optionm{\,(\agm{\,(\mathcal{P}(\vval))})})} \subseteq \Sigma$\hfill\mbox{}
\\[1mm]
\begin{minipage}[t]{\textwidth}
\small$\begin{array}{@{}l@{}l@{\;}l@{\;}l@{}}
S^\twoB_\Stack := \{
&  
\code{Stack.new}{:}
&
\forall P:\mathcal{P}(\vval).
&
\curlybracket{\lambda\,\argp\,\_\,\argo.\; \rplift{\argo = \opure\;\_ \lland \argp = \upcast{[]}}}
\\&
&&
\curlybracket{\lambda\,\retp\,\_.\; \exists \handle:\vptr.\; \rplift{\retp = \upcast{\handle}} * \isbag{\handle}{P}},
\\&
\code{Stack.push}{:}
&
\forall (\handle,v,P): \vptr \times \vval \ \ \ .
&
\curlybracket{\lambda\,\argp\,\_\,\argo.\; \rplift{\argo = \opure\;\_ \lland \argp = \upcast{[\handle, v]} \lland v\in P} * \isbag{\handle}{P}}
\\&
&\hspace*{3.2pc}{} \times \mathcal{P}(\vval)&
\curlybracket{\lambda\,\retp\,\_.\; \rplift{\retp \in \upcast{\vval}} * \isbag{\handle}{P}},
\\&
\code{Stack.pop}{:}
&
\forall (\handle,P): \vptr \times \mathcal{P}(\vval).
&
\curlybracket{\lambda\,\argp\,\_\,\argo.\; \rplift{\argo = \opure\;\_ \lland \argp = \upcast{[\handle]}} * \isbag{\handle}{P}}
\\&
&&
\curlybracket{\lambda\,\retp\,\_.\; \exists v:\vval.\; \rplift {\retp = \upcast{v} \lland (v = 0 \lor v \in P)} * \isbag{\handle}{P}}
\hfill\}
\end{array}$
\end{minipage}
\myhrule
\caption{Two abspecs on top of the first abstraction for the module \Stack{}}
\label{fig:stack2}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> hangul/draft_old <==
In this section, we first explain why contextual refinement is useful for modular verification, the essence of separation logic style reasoning, discuss challenges on combining them, and present our solution...

Background

(Say that we want to use contextual refinement for modular verification)
(앞에서 설명했다고 가정)

semantics. UB/NB, assume/guarantee 설명
(엄청 간단한 mutual sum)
(Hoare logic compile)
(앞에 논문 cite… 예제 가져와서...)

Hoare -> Sep
resource로... 내가 관측할 수 없는 영역에 대한 abstraction

[Module BWImpl]
local numFlip = 0

def get(): Int
  r = (numFlip%2 == 0) ? 0x000000 : 0xffffff
  return r

def flip(): Unit
  numFlip := numFlip + 1
  return ()

[BWHoare]
∀ is_black: bool, {{ own_half(is_black) }} get()  {{ r, own_half(is_black) * r = color_code(is_black) }}
∀ is_black: bool, {{ own_half(is_black) }} flip() {{ _, own_half(~is_black) }}
color_code \defeq …

[Client]
{{ own_half(true) }}
def main(): Unit
  {{ own_half(true) }}
  flip()
  {{ own_half(false) }}
  f() // f의 spec은 {{ True }} f {{ True }}
  {{ own_half(false) }}
  i := get()
  {{ own_half(false) * (i == color_code(false)) }}
  return i
목적: sep logic이 왜 필요한가? 가 아니고, (여기서) sep logic은 최대한 간단하게 설명하고 (뒤에서) 우리 challenge를 설명하는게 목적이다.

TODO: numFlip 그냥 boolean으로 하기 (예제는 simple할 수록 좋으니까)

직관을 말로 설명하고 (resource)
| half(b: bool) == token
| full(b: bool)
| undef
frame-preserving update 설명 (이 예시)

technically PCM... (일단 써보고 줄일 수 있으면 줄여보고) fp_update 정의가 위의 직관 어쩌구...



The key feature of modern separation logic is that it supports ownership (or more loosely speaking, knowledge) based reasoning. As an example, let us first take a look at the BWImpl module (figure 1) which consists of a module-local private (i.e., inaccessible from outside) variable numFlip, and two publicly accessible functions get and flip where the former returns color code of black or white depending on the parity of numFlip and the latter increments numFlip by one. Now, a reasonable specification for this module is written as Hoare Triples above (BWHoare). ...

token은 개념적으로...

Challenges

[Module BWSpecFail0]
def get(is_black: bool, tk: token): (Int, token)
  ...
//이런 식으로 해야 “계산” 가능해진다, 근데 문제는 CR 깨짐
//교수님 슬라이드에서 Take 만 인자로. (state 계산해서 넣고 이런건 그대로)

[Module BWSpecFail1]
def get(): Int
  is_black := choose()
  tk := choose()
  ...

물리적으로 관측 안되는 값을…
가능한 spec 써보고 왜 안되는지 설명
P Q를 정확하게 인코딩하는 함수를 쓸 수 있는가
Explain challenges - (1) argument passing breaks contextual refinement, (2) just choosing a random value is not appropriate.
get이 물리적 값하고 연관이 있으니... get 먼저 설명하는게 더 나을 듯
logical argument 없는데 부르는거
f가 flip 을 부르는 경우에도 refinement 성립 (separation logic은 그런 경우가 없다고 가정하는 것이고…)
type checker

Solutions

주는 사람이 없기 때문에, 뭐를 주던 ...
Key idea is “Take” operation -- give a glimpse to our solution.
어느정도 technical하게 일단 쓰고…
(c = Take Bool) 5가지 케이스 다 한거고 4가지는 UB
(Q: 1가지로 deterministic한거 아니냐? Take 꼭 필요하냐? ---> 이렇게까지 이야기 안해도 이해할 수 있을 듯)

reasoning은 했지만... assume이 이렇게 많은데 UB 뜰 수 있으면 의미없는 spec.
Type Checker이야기!

Formally define choose/take, UB/NB, assume/guarantee.
UB is erroneous, NB is partial termination...
Before presenting our solution in detail, explain more about separation logic proof (what is going on under the hood) -- PCM, invariants, etc.

[Module BWSpec]
def get(): Int
  ...

def flip(): Unit
   ...

Now present our solution. [dependency: PCM, choose/take, assume/guarantee, UB/NB]



















==> hangul/echo <==
사용자에게는 (echo_white []) 만 usable로 정의하고, echo_get/put은 숨기고 싶음 -- static 함수
--------------------------------------------------------------------------
{{ echo_white [] }}
def echo(): Unit
  let stk: list Int64 := echo_get([]);
  echo_put(stk)
{{ echo_white [] }}
--------------------------------------------------------------------------
{{ echo_white stk }}                        // the same "stk" with varg
def echo_get(stk: list Int64): list Int64
  {{ echo_white stk }}
  let n = getint();
  {{ echo_white stk }}
  if(n == -1) {
    {{ echo_white stk }}
    return stk;
  }
  {{ echo_white (n :: stk) }}
  let ret := echo_get((n :: stk));
  {{ echo_white ret }}
  return ret
{{ echo_white ret }}                        // the same "stk" with vret
--------------------------------------------------------------------------
{{ echo_white stk }}                        // the same "stk" with varg
def echo_put(stk: list Int64): Unit
  match stk with
  | [] => return ()
  | n :: stk' =>
    putint(n);
    echo_put(stk')
  end
{{ echo_white stk }}                        // the same "stk" with varg

sim rel: ∃ xs, is_stack mp_tgt xs /\ Own(echo_black xs) /\ forall x in xs, x <> -1





만약 echo_black/white 두개가 있는게 아니라 echo_excl 하나만 있으면?
- getint() 다녀와도 xs 값이 안변했다는 것을 알아야 하는데 이게 잘 안됨
  (precond에 echo_excl 요구해야 하니까 sim_rel에는 echo_excl 못넣음.
   그러면 call 다녀왔을 때 xs가 아무거나로 바뀌어있을 수 있음.)

private transition이 있었다면 echo_excl 하나만으로도 가능할 듯
- le := excl 가지고 있으면 xs 불변, 아니면 top2
  lepriv := excl 넣고 빼고 허용



static 키워드 관련
- Imp lang에 지금 없나...? 어떻게 안되나?
- Spec에서는 Stb에 자기가 publish 안하면 되는거다?


==> hangul/intro-example <==

#+BEGIN_EXAMPLE
```
def new(): Ptr
  Ptr stk = alloc(1);
  return stk

def push(Ptr stk, Int64 n): Unit
  let new_node := alloc(2);
  store(new_node, 0, n);
  let hd := load(stk, 0);
  store(new_node, 1, hd);
  store(stk, 0, new_node);
  debug(true, n);
  return ()

def pop(Ptr stk): Int64
  let hd := load(stk, 0);
  if(ptrcmp(hd, NULL) != 0) {
    let v    := load(hd, 0);
    let next := load(hd, 1);
    free(hd, 2);
    store(stk, 0, next);
    debug(false, v);
    return v
  }
  debug(false, -1);
  return -1
```

Module Stack {
  local stk_mgr: Ptr -> option (list Int64) = fun _ => None

  def new(): Ptr
    let handle := Choose(Ptr);
    guarantee(stk_mgr(handle) = None);
    stk_mgr(handle) := Some [];
    return handle

  def push(handle: Ptr, x: Int64): Unit
    let stk := unwrap(stk_mgr(handle));
    stk_mgr(handle) := Some (x :: stk);
    debug(true, x);
    ()

  def pop(handle: Ptr): Int64
    let stk := unwrap(stk_mgr(handle));
    match stk with
    | x :: stk' => 
      stk_mgr(handle) := Some stk';
      debug(false, x);
      return x
    | [] => return -1
    end
}

```
is_stack (handle: Ptr) (xs: list Int64): iProp := ...

                                       {{ }} new()           {{ stk0. (stk0 = []) ** ∃ handle, is_stack handle stk0 }}
∀ handle stk0,    {{ is_stack handle stk0 }} push(handle, x) {{ stk1. (stk1 = x ::= stk0) ** is_stack handle stk1 }}
∀ handle stk0,    {{ is_stack handle stk0 }} pop(handle)     {{ (x, stk1). match stk0 with
                                                                           | [] => (x = -1) ** (stk1 = []) ** is_stack handle stk1
                                                                           | hd :: tl => (x = hd) ** (stk1 = tl) ** is_stack handle stk1
                                                                           end }}

new_body(): List Int64                           := return [];
push_body(stk: List Int64, x: Int64): List Int64 := (debug(true, x); return (x :: stk))
pop_body(stk: List Int64): (Int64, List Int64)   := (match stk with 
                                                     | [] => return (-1, [])
                                                     | x :: xtl => debug(false, x); return (x, xtl)
                                                     end)

TTTTTTTTTTTTTTTTTTTTTTTODO: pop_body인자 xs는 forall에서 온거라 치는데 ret이 매치가 안됨. 위 spec 지금 타입 안맞음


          new_body() := (let ret := Choose _; return ret)
push_body(handle, x) := (let ret := Choose _; debug(true, x); return ret)
    pop_body(handle) := (let ret := Choose _; debug(false, ret); return ret)




------------------------------------------------------------------------------------------------------

#### debug도 non-det하게 choose하는데 P 만족하게 guarantee 해서 넣기

is_stack_shared (handle: Ptr) (P: Int64 -> Prop): iProp := ...
                                           ∀ P, {{ }} new()           {{ handle, is_stack_shared handle P }}
∀ handle P x, {{ (P x) ** is_stack_shared handle P }} push(handle, x) {{ _,      is_stack_shared handle P }}
∀ handle P,            {{ is_stack_shared handle P }} pop(handle)     {{ ret,    is_stack_shared handle P ** (ret = -1 \/ exists hd, P hd /\ ret = hd) }}
```
#+END_EXAMPLE

==> hoare-logic.tex <==
\subsection{Hoare logic specifications in \CREMS{}}
\label{sec:overview:hoare}

To demonstrate how to express Hoare logic~(HL) specifications in \CREMS,
consider the implementations $I_\code{Main}$ and $I_\code{F}$ of the modules \Main{} and \MF{}, shown in \Cref{fig:hoare-logic}.
Here \code{Main.main()} $(i)$ invokes \code{F.f(x)} with $\code{x} = 40$, which computes \code{x*x/4+x+1}, prints it out via the system call \prt{} and returns it;
$(ii)$ if the result is an odd number, prints \code{42}; $(iii)$ otherwise, crashes by executing division by zero.
In HL, the specification $S_\Main$ says that \code{Main.main()} runs safely, \emph{assuming} the specification $S_\MF$,
which says that if the argument of \code{F.f} is a multiple of \code{4}, it runs safely and returns a number $r$ such that $r$ modulus \code{4} is {1}.

In \crems, assuming the specifications $S_\code{Main}$ and $S_\code{F}$ (ignoring the safety), we would like to \emph{locally} verify $I_\code{Main}$ and $I_\code{F}$ against, \eg the abstractions $A_\code{Main}$ and $A_\code{F}$ in \Cref{fig:hoare-logic}, where the abstracted parts are \fbox{boxed} and \code{**} is the exponentiation operator.
First, note that without any assumption neither $I_\code{Main} \lectx A_\code{Main}$ nor $I_\code{F} \lectx A_\code{F}$ holds
because their context implementations are arbitrary.
For example, \code{0} may be given for \code{r} in $\code{Main.main()}$, and \code{1} may be given for \code{x} in $\code{F.f(x)}$, in which cases the implementation and abstraction behave differently.
The question here is how to \emph{internalize} the specifications inside $A_\code{Main}$ and $A_\code{F}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{figures/hoare-logic}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The abspecs $\spcmod{S_\code{Main} \cup S_\code{F}}{A_\code{Main}}{S_\code{Main}}$ and $\spcmod{S_\code{Main} \cup S_\code{F}}{A_\code{F}}{S_\code{F}}$
internalizing $S_\code{Main},S_\code{F}$ inside $A_\code{Main}$ and $A_\code{F}$ are given in \Cref{fig:hoare-logic},
where we simply insert \kwassume{} and \kwguarantee{} commands according to $S_\code{Main}$ and $S_\code{F}$.
Specifically, \code{F.f(x)} \emph{assumes} its precondition \code{x\%4 == 0} at the beginning and \emph{guarantees} its postcondition \code{r\%4 == 1} at the end.
Conversely, \code{Main.main()} \emph{guarantees} the precondition of \code{F.f(x)} before invoking it and
\emph{assumes} the postcondition of \code{F.f(x)} after the invocation.
Note that we simply omitted \code{\kwassume(true)} and \code{\kwguarantee(true)} corresponding to $\hoare{\TRUE}{}{\TRUE}$ of \code{Main.main()}
because they do nothing as we will see below.

Now the computational interpretation of \kwassume{} and \kwguarantee{} is given as follows.
First, $\kwassume(P)$ for a proposition $P$ does nothing if $P$ holds; otherwise triggers \emph{undefined behavior (UB)}, which is a standard notion (\eg in CompCert) and interpreted as exhibiting all possible behaviors:
\[
\kwassume(P) ~\defeq~ \code{\kwif{} $P$ \kwthen{} \kwskip{} \kwelse{} \kwub{}}
\]
To see the intuition, consider proving $I_\code{F} \lectx \spcmod{S_\code{Main} \cup S_\code{F}}{A_\code{F}}{S_\code{F}}$.
If the argument \code{x} to \code{F.f} does not satisfy \code{x\%4 == 0}, the abspec triggers \kwub{} thereby exhibiting all possible behaviors, which trivially include whatever behavior the implementation may exhibit.
Therefore in the verification we do not need to consider the cases where the assume command fails (\ie we can assume it holds).

Second, $\kwguarantee(P)$ does nothing if $P$ holds; otherwise triggers \emph{no behavior (NB)}, which appeared in~\cite{compcerttso, int2ptr} and is interpreted as exhibiting no behaviors (see \Cref{sec:formal} for the formal definition):
\[
\kwguarantee(P) ~\defeq~ \code{\kwif{} $P$ \kwthen{} \kwskip{} \kwelse{} \kwnb{}}
\]
Again, for $I_\code{F} \lectx \spcmod{S_\code{Main} \cup S_\code{F}}{A_\code{F}}{S_\code{F}}$, suppose the argument \code{x} satisfies \code{x\%4 == 0}
and then both implementation and abspec will compute and print the same value \code{r}.
Now if \code{r} does not satisfy \code{r\%4 == 1}, the abspec triggers \kwnb{} thereby exhibiting no behaviors, which does not include whatever behavior the implementation may exhibit (unless it also triggers \kwnb{}, which is not the case here).
Therefore in the verification we must prove that the guarantee command succeeds (\ie we should guarantee it holds).

Then, we can actually prove $I_\code{Main} \lectx \spcmod{S_\code{Main} \cup S_\code{F}}{A_\code{Main}}{S_\code{Main}}$
and $I_\code{F} \lectx \spcmod{S_\code{Main} \cup S_\code{F}}{A_\code{F}}{S_\code{F}}$.
For the former, we first prove \code{\kwguarantee(x\%4 == 0)} succeeds since \code{x} is \code{40}; then for any given \code{r} from \code{F.f(x)},
we can assume \code{r\%4 == 1}, which implies \code{r\%2 == 1} thereby proving that both implementation and abspec print \code{42}.
For the latter, we can assume \code{x\%4 == 0} thereby proving that both implementation and abspec compute and print the same value \code{r}.
Then \code{\kwguarantee(r\%4 == 1)} succeeds since \code{r} is \code{(x/2 + 1)**2} and we assumed \code{x\%4 == 0}.
Finally, both return the same \code{r}.

Finally, we can see that the following hold:
\[
  \beh{\spcmod{S_\code{Main} \cup S_\code{F}}{A_\code{Main}}{S_\code{Main}} \link \spcmod{S_\code{Main} \cup S_\code{F}}{A_\code{F}}{S_\code{F}}} \subseteq \beh{A_\code{Main} \link A_\code{F}}
\]
which easily follows using the following lemma: for any proposition $P$ and any program with a hole $K[-]$,
\[
\beh{K[\kwguarantee(P); \kwassume(P)]} \subseteq \beh{K[\kwskip]}
\]
This lemma holds trivially if $P$ holds; otherwise it holds since the left hand side exhibits no behavior.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> proofmode.tex <==
\section{Proofmode}
\label{sec:proofmode}

\crems proof mode consists of two modes supporting simulation reasoning and separation logic reasoning.

\subsection{Simulation Reasoning}

\myparagraph{Reduction Tactics}
We establish CR using a simulation technique,
which relates an implementation state and an abspec state\footnote{
  In fact, our simulation tactics generally work for relating \emph{any} two \ems{} semantics.
}.
%% both of which consist of an itree with a module-local state.
To take steps,
we provide reduction tactics that reduces
the current itree (either in implementation or in abspec) into the head normal form
by, \eg converting $(i \mbind j) \mbind k$ into $i \mbind (j \mcat k)$.
Also, we made the tactics extensible:
when embedding a new language with new effects and a new handler H into \ems{},
we can register new reduction lemmas about H
so that they are used by the reduction tactics
(\eg converting $H(i \mbind j)$ into $H i \mbind H j$).

\myparagraph{Simulation Tactics}
We provide tactics that automate common parts of simulation reasoning.
Specifically, the tactics repeatedly apply the rules given below (\ie converting the conclusion into the premise),
where we omitted the state component and the world index in the simulation relation for brevity.
%% \footnote{Note that establishing the relational invariant is only required at the interaction points, not in between.}.
Note that the \dashbox{dash-boxed} rules are \emph{complete} (\ie the premise and conclusion are equivalent) while the others not.
%% --- in a sense that it does not mistakenly yields an unprovable goal ---
%% and the others not.
Then we provide three tactics:
\kw{steps} automatically applies complete rules as many as possible,
\kw{force\_i} applies any available rule once in the implementation side,
and 
\kw{force\_a} does the same for the abspec side.
\[
\scriptsize
\begin{array}{c@{\quad}c@{\quad}c@{\quad}c}
\infer{\exists x \in X.~T_\iside \lesssim K_\aside[x]}
      {T_\iside \lesssim \code{x := \kwchoose($X$); $K_\aside[\code{x}]$}} &
\dashbox{
\infer{\forall x\in X.~ T_\iside \lesssim K_\aside[x]}
      {T_\iside \lesssim \code{x := \kwtake($X$); $K_\aside[\code{x}]$}}} &
\infer{P \lland (T_\iside \lesssim T_\aside)}
      {T_\iside \lesssim \code{\kwguarantee($P$); $T_\aside$}} &
\dashbox{
\infer{P \implies T_\iside \lesssim T_\aside}
      {T_\iside \lesssim \code{\kwassume($P$); $T_\aside$}}}
\\

\span\\

\dashbox{
\infer{\forall x\in X.~ K_\iside[x] \lesssim T_\aside}
      {\code{x := \kwchoose($X$); $K_\iside[\code{x}]$} \lesssim T_\aside}} &
\infer{\exists x\in X.~ K_\iside[x] \lesssim T_\aside}
      {\code{x := \kwtake($X$); $K_\iside[\code{x}]$} \lesssim T_\aside} &
\dashbox{
\infer{P \implies T_\iside \lesssim T_\aside}
      {\code{\kwguarantee(P); $T_\iside$} \lesssim T_\aside}} &
\infer{P \lland (T_\iside \lesssim T_\aside)}
      {\code{\kwassume(P); $T_\iside$} \lesssim T_\aside}
\\
\end{array}
\]

%% \begin{figure}[h]

%% \footnotesize
%% \[
%% \begin{array}{c@{\qquad\qquad}c}
%% \dashbox{
%% \infer{\forall x, K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {\code{\kwvar{} x := \kwchoose($X$); $K_{tgt}[\code{x}]$} \lesssim K_{src}}} &
%% \infer{\exists x, K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {K_{tgt} \lesssim \code{\kwvar{} x := \kwchoose($X$); $K_{src}[\code{x}]$}}
%% \\

%% \span\\

%% \infer{\exists x, K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {\code{\kwvar{} x := \kwtake($X$); $K_{tgt}[\code{x}]$} \lesssim K_{src}} &
%% \dashbox{
%% \infer{\forall x, K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {K_{tgt} \lesssim \code{\kwvar{} x := \kwtake($X$); $K_{src}[\code{x}]$}}}
%% \\

%% \span\\

%% \dashbox{
%% \infer{P \implies K_{tgt} \lesssim K_{src}}
%%       {\code{\kwguarantee(P); $K_{tgt}$} \lesssim K_{src}}} &
%% \infer{P \land K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {K_{tgt} \lesssim \code{\kwguarantee($P$); $K_{src}$}}
%% \\

%% \span\\


%% \infer{P \land K_{tgt} \lesssim K_{src}}
%%       {\code{\kwassume(P); $K_{tgt}$} \lesssim K_{src}} &
%% \dashbox{
%% \infer{P \implies K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {K_{tgt} \lesssim \code{\kwassume($P$); $K_{src}$}}}
%% \\
%% \end{array}
%% \]

%% \hspace*{-1.5cm}
%% \begin{minipage}{1.2\textwidth}
%% \small
%% \[
%% \begin{array}{c@{\quad}c@{\quad}c@{\quad}c}
%% \infer{\forall x, K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {\code{x := \kwchoose($X$); $K_{tgt}[\code{x}]$} \lesssim K_{src}} &
%% \infer{\forall x, K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {\code{x := \kwchoose($X$); $K_{tgt}[\code{x}]$} \lesssim K_{src}} &
%% \infer{\forall x, K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {\code{x := \kwchoose($X$); $K_{tgt}[\code{x}]$} \lesssim K_{src}} &
%% \infer{\forall x, K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {\code{x := \kwchoose($X$); $K_{tgt}[\code{x}]$} \lesssim K_{src}}
%% \\

%% & \\

%% \infer{\forall x, K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {\code{x := \kwchoose($X$); $K_{tgt}[\code{x}]$} \lesssim K_{src}} &
%% \infer{\forall x, K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {\code{x := \kwchoose($X$); $K_{tgt}[\code{x}]$} \lesssim K_{src}} &
%% \infer{\forall x, K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {\code{x := \kwchoose($X$); $K_{tgt}[\code{x}]$} \lesssim K_{src}} &
%% \infer{\forall x, K_{tgt}[\code{x}] \lesssim K_{src}}
%%       {\code{x := \kwchoose($X$); $K_{tgt}[\code{x}]$} \lesssim K_{src}}
%% \\
%% \end{array}
%% \]
%% \end{minipage}

%% \caption{Commonly used simulation rules (simplified).}
%% \label{proofmode:sim}
%% \end{figure}

\subsection{Separation Logic Reasoning}
%% \begin{figure}[h]
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% $P, Q ::= \forall x, P \;|\; \exists x, P \;|\; \lc P \rc \;|\;
%%   P \land Q \;|\; P \lor Q \;|\; P \Rightarrow Q \;|\;
%%    P * Q \;|\; P \wand Q \;|\;
%%   \ownGhost{}{a: \Sigma} \;|\; \upd{} P \;|\; P \vdash Q
%%   $
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% \label{proofmode:iprop}
%% \caption{Instantiated Iris connectives.}
%% \end{figure}
\[
\forall x.\; P \;|\; \exists x.\; P \;|\; \lc P \rc \;|\;
P \land Q \;|\; P \lor Q \;|\; P \Rightarrow Q \;|\;
P * Q \;|\; P \wand Q \;|\;
\ownGhost{}{a: \Sigma} \;|\; \upd{} P \;|\; P \vdash Q
\]
%% SL tactics works when the source module is abspec and
%% SL tactics support $\rProp$-level reasoning.
%% (presented above) and their rules,
%% which in turn allows us to use IPM (Iris Proof Mode) when
%% proving logical entailment.
We support the SL tactics provided by IPM (Iris Proof Mode).
For this, we define the standard \iris connectives shown above on $\rProp$, instead of $\mathbf{iProp}$ of \iris with step indices,
and prove the lemmas that IPM (Iris Proof Mode) requires, which allows us to use IPM when proving logical entailment.
Note that we omitted the later modality ($\latert$) because we do not use step-indexing.

\myparagraph{At Interaction Points}
We have three tactics -- \kw{slinit}, \kw{slcall}, and \kw{slret} -- for each interaction
points. \kw{slinit} is used at the beginning of a function and it moves the precondition (in $\rProp$)
into Coq hypothesis (\code{current\_rProps}).
%% \begin{samepage}
%% \begin{shaded}
%% \begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\small]
%% H: current\_rProps [("R1":$\exists\,x,P\,x$); ("R2":$\upd{}\ownGhost{}{\mires}$); $\ldots \;]$
%% ----------------------------------------------------- (1/1) // Coq Turnstile
%% ... // simulation goal
%% \end{Verbatim}
%% \end{shaded}
%% \end{samepage}
%% SRC: SL\_call $S_{all}$ fname args >>= ...
%% TGT:    call    $\,$ fname args >>= ...
%% \noindent
\kw{slcall} is used when calling a function ---
where source have its call decorated with \code{\AS\_call} (\Cref{formal:embedding2}) and
target not. It asks the user to specify a subset of \code{current\_rProps} that will be
consumed when proving (with IPM) both (i) callee's precondition and (ii) the relational
invariant. After that, the user proceeds the proof with fresh \trm{rProp}s satisfying (i)
callee's postcondition and (ii) the relational invariant. In other words, while the mechanism
is implemented with various \kwassume{}/\kwguarantee{}s in low-level (\eg \code{\AS\_call}), we
give a high-level interface with these tactics. \kw{slret} is used at the end of the function
and is similar to \kw{slcall}.

%% (according to the callee's precondition)
%% Note that, Most of the time (i-iv) will be specified by wildcard patterns.
%% (i) a meta-variable, (ii) an optional ordinal number, (iii) virtual arguments, and most importantly, (iv)


\myparagraph{In Between} We also support operations on \code{current\_rProps} in the middle
of the simulation proof. Notably, we support (i) eliminating connectives like $\forall,
\exists, \lor, \land, *, \upd{}, \lc \rc$, (ii) \kw{Assert} tactic that consumes specified
\trm{rProp}s to establish specified goal (using IPM), and (iii) \kw{OwnV} tactic that gives
$\wdef(\mires)$ for given $\ownGhost{}{\mires}$.  It is worth noting that, despite such
functionalities, it suffices to put updates and validity checking only at the interaction
points (as in \Cref{sec:overview:separation}), not in between.

%% \kw{Assert $P$ with "$R_{1} \ldots R_{n}$"} tactic that consumes $R_{1} \ldots R_{n}$ from current \trm{rProp}s to establish $P$,
%% (iii) \kw{Assert $P$ with "$R_{1}$ ... $R_{n}$"} tactic that consumes "A", \ldots, "B" from current \trm{rProp}s to establish $P$, and


%% It is technically the most intricate part and required a slight generalization (compared to
%% \Cref{sec:overview:separation}) shown in formal section. Note however that, as in
%% \Cref{sec:overview:separation}, it suffices to put \kwfpu{} and validity checking only at the
%% interaction points (not in between).




%% \begin{lcverbatim}
%% current_iProps: "P": True, "Q": False
%% ------------------------------------------ (1/1)
%% \end{lcverbatim}


==> sep-logic.tex <==
\subsection{Separation logic specifications in \CREMS{}}
\label{sec:overview:separation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{figures/sep-logic}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Now to see how we can express separation logic (SL) specifications in \CREMS,
consider the implementations $I_\Cannon$ and $I_\Main$  of the two modules \Main{} and \Cannon{}, shown in \Cref{fig:sep-logic}.
Here \code{\Main{}.\main{}()} invokes \code{\Cannon{}.\fire{}()} and prints the return value for a fixed number, \numfire{}, of times.
The \Cannon{} module consists of $(i)$ the \emph{module-local} variable \powder{} (\ie not accessible to other modules),
which is initially set to \code{1} and
$(ii)$ the function \fire{}, which sets the variable \code{r} to be \code{1/\powder{}}, prints \code{r}, decrements \powder{} by \code{1}, and returns \code{r}.
Note that \code{\Cannon{}.\fire{}()} can be safely invoked only once because it will crash due to division by zero at the second invocation;
therefore, if \numfire{} is \code{2}, the whole program crashes.

We briefly discuss how one can prove safety of the program when \numfire{} is \code{1} in SL.
First, the SL specification $S_\Cannon$ (given in \Cref{fig:sep-logic}) says that
if the resource $\ball$ is logically given, \code{\Cannon{}.\fire{}()} safely executes and returns \code{1}
but does not logically give the $\ball$ back (\ie $\ball$ is \emph{consumed}).
Here one can intuitively understand a \emph{resource} as something that is neither duplicable nor creatable out of nothing.
In this example, we can design the universe of resources---via a general mechanism based on PCMs (Partial Commutative Monoids)---in such a way that there can be at most one $\ball$,
relying on which we can then \emph{locally} prove the safety of \code{\Cannon{}.\fire{}()}
since it requires $\ball$ and thus can be invoked at most once.
Second, the SL specification $S_\Main$ says that given a $\ball$, \code{\Main{}.\main{}()} safely executes,
which is \emph{locally} provable relying on $S_\Cannon$ since \numfire{} is \code{1} and thus \code{\Cannon{}.\fire{}()} is invoked only once.
Indeed, if \numfire{} was \code{2}, one cannot verify \code{\Main{}.\main{}()} against $S_\Main$
since there is no $\ball$ left at the second invocation of \code{\Cannon{}.\fire{}()}.
Note that this kind of reasoning would not be possible in Hoare logic because
\code{\Cannon{}.\fire{}()} has no arguments, so that it would be hard to express any kind of precondition.

With this intuition, in \crems, assuming $S_\Main$ and $S_\Cannon$, we would like to \emph{locally} verify $I_\Main$ and $I_\Cannon$ against, \eg the abstractions $A_\Main$ and $A_\Cannon$ in \Cref{fig:sep-logic}, where the abstracted parts are \fbox{boxed}.
Note that without any assumption neither $I_\Main \lectx A_\Main$ nor $I_\Cannon \lectx A_\Cannon$ holds
since their context modules are arbitrary and hence, \eg \code{0} may be given for \code{r} in $\code{Main.main()}$, and also
\code{\Cannon{}.\fire{}()} may be invoked twice by the context in which case $I_\Cannon$ crashes but $A_\Cannon$ runs successfully.
As before, to solve this problem, we will \emph{internalize} the SL specifications inside the abstractions,
which are the abspecs given in \Cref{fig:sep-logic}:
\[
\spcmod{S_\Main \cup S_\Cannon}{(A_\Main,\mires_\Main)}{S_\Main} \text{ and }
\spcmod{S_\Main \cup S_\Cannon}{(A_\Cannon,\mires_\Cannon)}{S_\Cannon}
\]

To understand the abspecs, we first see how the set of resources $\kwcanonpcm$ is defined.
Concretely, $\kwcanonpcm$ consists of five elements $\kwundef, \kwemp, \ready, \fired, \ball$ with a commutative binary operator $+$ defined as follows:
\begin{itemize}
\item $\forall p \in \kwcanonpcm,~ \kwundef + p = \kwundef$
\item $\forall p \in \kwcanonpcm,~ \kwemp + p = p$
\item $\ready + \ball = \fired$
\item $\fired + \ready = \fired + \ball = \ready + \ready = \fired + \fired = \ball + \ball = \kwundef$
\end{itemize}
The intuition here is that $\kwundef$ represents undefinedness (\ie \emph{inconsistency}); $\kwemp$ the \emph{empty resource}, which is the identity for $+$;
$\ready$ the \emph{knowledge} that \Cannon{} is not yet fired;
$\fired$ that \Cannon{} is already fired;
and $\ball$ the \emph{capability} to invoke \code{\Cannon{}.\fire{}()}.
The definition of $+$ captures that only a subset of $\{\ready, \ball\}$ or $\{\fired\}$ is consistent; in particular,
there cannot be two (or more) \ball{s} since $\ball + \ball = \kwundef$.

Now we look at the abspecs.
The dotted boxes are generated from $S_\Main$ and $S_\Cannon$,
where \ASSUME{} and \GUARANTEE{} are the macros defined at the bottom of \Cref{fig:sep-logic}.
Also the \boilerplate{gray code} is boilerplate
and the \hl{highlighted parts} are modules' initial resources, which come from $\mires_\Main$ and $\mires_\Cannon$ of the abspecs.

Then we see how it works.
Each module has a module-local resource, \mres, initialized with its initial resource
and each function has a function local resource, \lres, initialized with \kwemp{}.
Then \code{\Cannon.\fire{}()} \emph{assumes} its precondition saying that a resource \ball{} is given at the beginning, and \emph{guarantees} its postcondition saying that no resource is returned and the return value \code{r} is \code{1} at the end.
\code{\Main.\main{}()} also \emph{assumes} its precondition saying that a resource \ball{} is given at the beginning; then \emph{guarantees} the precondition of \code{\Cannon.\fire{}()} before invoking it and \emph{assumes} the postcondition of \code{\Cannon.\fire{}()} after the invocation;
finally \emph{guarantees} its postcondition at the end.

Now we see the computational interpretation of \ASSUME{} and \GUARANTEE{}, whose macro definitions are given in \Cref{fig:sep-logic}.
First, \textcolor{red}{\code{\ASSUME(Cond)}} \emph{takes} a resource; assumes it satisfies \code{Cond};
adds it to \lres{}; and assumes \lres{} is consistent with \mres{}.
Here the \kwtake{} operation is a key technique in \crems and will be explained below.
For now, we simply consider as if \code{\kwtake(\kwcanonpcm)} magically takes the resource that is given by the caller or returned by the callee.
%
Second, \textcolor{blue}{\code{\GUARANTEE(Cond)}} $(i)$ nondeterministically updates \mres{} and \lres{} via \kwfpu{}, called \emph{frame-preserving update (FPU)}\footnote{
  The notion of frame-preserving update comes from modern separation logic such as \iris~\cite{irisgroundup}.
};
$(ii)$ nondeterministically \emph{chooses} a resource; $(iii)$ guarantees it satisfies \code{Cond}; and $(iv)$ \emph{subtract} it from \lres{}.
In $(i)$, we are allowed to update the module and function resources before jumping to another function,
which however is restricted to FPUs. The definition of \kwfpu{} is given as follows\footnote{
  Our formal definition of $\kwfpu$ is slightly more general as found in SLs (see \Cref{formal:embedding2} for details).
}:
\[
\begin{array}{@{}l@{}}
  \kwfpu(\mres,\lres) ~\defeq~ \kwchoose(\{ (\mres',\lres') \,|\, \forall \resframe \in \kwcanonpcm,~ \\
  \hspace*{1pc}\code{\resframe + $\mres$ + $\lres$ != \kwundef} \implies \code{\resframe + $\mres'$ + $\lres'$ != \kwundef} \})
\end{array}
\]
where $\kwchoose(X)$ nondeterministically picks an element from the given set $X$.
The intuition is that one can update $\mres$ and $\lres$ in such a way that consistency is preserved
under an arbitrary frame resource $\resframe$ (capturing possible resources remaining in other modules).
In $(ii)$, although a resource $\res$ is just nondeterministically chosen,
for now we simply consider as if it is magically passed to the callee or returned to the caller.
In $(iii)$, if the chosen $\res$ does not satisfy the condition $\code{Cond}$, it triggers no behavior,
which means that only that resource satisfying the condition can be chosen.
In $(iv)$, we performed the subtraction because we are passing it to another function, which will add it to its own function resource as we have seen above in \textcolor{red}{\code{\ASSUME(Cond)}}.
The definition of $\kwminus$ is given as follows:
\[
  \kwminus(\lres,\res) ~\defeq~ \kwchoose(\{ \lres' \,|\, \code{$\lres'$ + $\res$ == $\lres$} \})
\]
Note that when there is no such $\lres'$, it triggers no behavior because choosing from the empty set does so.

%% \minki{Add footnote? physical하게 resource를 넘기도록 했고 그렇기 때문에 contextual refinement가 안 되는 work: \cite{steelcore}}
Now we see how the illusion of resource passing between functions works via \kwchoose{} and \kwtake{}.
First of all, note that it does not make sense to \emph{physically} pass any resource information to context modules or receive it from them
because context modules are completely arbitrary and thus may not understand such resource information (\eg those written in \imp).
%% we cannot physically pass any resource information across modules
Our key observation, however, is that by defining \kwtake{} as the dual operation to \kwchoose{}, we can logically make such an illusion.
Specifically, the nondeterministic choice \kwchoose{} and its dual \kwtake{}\footnote{
  The dual to (standard or demonic) nondeterminism is called \emph{angelic nondeterminism} in the literature~\cite{bodik2010programming, back2012refinement, tyrrell2006lattice, jeremie:lics}.
} are defined as follows for any set $X$ (See \Cref{sec:formal} for formal definitions).
\[
\begin{array}{rcl}
  \beh{\code{x := \kwchoose($X$); $K[\code{x}]$}} &\defeq& \bigcup_{x\in X} \beh{K[x]} \\
  \beh{\code{x := \kwtake($X$); $K[\code{x}]$}} &\defeq& \bigcap_{x\in X} \beh{K[x]} \\
\end{array}
\]
Note that $\kwchoose(\emptyset)$ is NB and $\kwtake(\emptyset)$ is UB.
The intuition is that
when proving $\beh{I} \subseteq \beh{\code{\res := \kwchoose(\kwcanonpcm); $K[\res]$}}$,
it suffices to prove $\beh{I} \subseteq \beh{K[\res]}$ for \emph{some} resource $\res$,
which allows us to \emph{logically} (\ie in the proof) pick a particular resource to pass to the context.
On the other hand,
when proving $\beh{I} \subseteq \beh{\code{\res := \kwtake(\kwcanonpcm); $K[\res]$}}$,
we need to prove $\beh{I} \subseteq \beh{K[\res]}$ for \emph{every} resource $\res$,
which makes sense
because we do not know what resource will be given from the context, and thus we have to prove the refinement whatever resource is given.
Then we have the following theorem, which makes the illusion of passing a resource from \kwchoose{} to \kwtake{}.
\begin{equation}
\begin{array}{@{}rl@{}}
&\beh{\code{\res{} := \kwchoose(\kwcanonpcm); $K[\res]$; $\res'$ := \kwtake(\kwcanonpcm); $K'[\res']$}}\\
\subseteq
&\beh{\code{\res{} := \kwchoose(\kwcanonpcm); $K[\res]$; $K'[\res]$}}
\end{array}\tag{$\star$}
\end{equation}
This theorem holds simply by instantiating the \kwtake{} operation with the chosen resource $\res$.

With this, we can prove $I_\Main \lectx \spcmod{S_\Main \cup S_\Cannon}{(A_\Main,\mires_\Main)}{S_\Main}$ for ${\numfire = 1}$.
When $\Main.\main()$ is invoked,
by \textcolor{red}{\code{\ASSUME($\lambda$\res. \res{} == \ball)}}
for any \emph{taken} resource $\res$, we can assume \code{\res{} == \ball} and thus add $\ball$ to $\lres$ yielding $\ball$.
Then
for \textcolor{blue}{\code{\GUARANTEE($\lambda$\res{}. \res{} == \ball)}}
the abspec does not update \mres{}, \lres{}, \emph{chooses} $\ball$ for $\res$ to satisfy the precondition of $\Cannon.\fire()$,
and successfully subtracts $\ball$ from $\lres$ yielding $\kwemp$.
Then both implementation and abspec invoke $\Cannon.\fire()$ and receive the same return value \code{r}.
By \textcolor{red}{\code{\ASSUME($\lambda$\res{}. \res{} == \kwemp \&\& r == 1)}}
for any \emph{taken} resource $\res$, we can assume \code{\res{} == \kwemp \&\& r == 1}, and thus add $\kwemp$ to $\lres$ yielding $\kwemp$.
Since $\code{r} = 1$, both implementation and abspec print \code{1}.
Finally,
we can trivially satisfy \textcolor{blue}{\code{\GUARANTEE($\lambda$\res{}. \res{} == \kwemp)}}
by not updating the module and function resources and \emph{choosing} $\kwemp$ for $\res$.
It is important to note that for ${\numfire = 2}$ the above proof breaks down
since at the second iteration we do not have $\ball$ anymore and thus cannot satisfy
\textcolor{blue}{\code{\GUARANTEE($\lambda$\res{}. \res{} == \ball)}}.

Similarly, we can prove $I_\Cannon \lectx \spcmod{S_\Main \cup S_\Cannon}{(A_\Cannon,\mires_\Cannon)}{S_\Cannon}$.
This time we set the module-local relational invariant to be $(\powder = 1 \land \mres = \ready) \lor (\powder = 0 \land \mres = \fired)$, which initially holds.
Then when $\Cannon.\fire()$ is invoked,
by \textcolor{red}{\code{\ASSUME($\lambda$\res{}. \res{} == \ball)}}
for any \emph{taken} resource $\res$, we can assume \code{\res{} == \ball} and thus add $\ball$ to $\lres$ yielding $\ball$.
Now due to the relational invariant, we have two cases.
First, when $\powder = 0 \land \mres = \fired$, the refinement trivially holds since $\mres + \lres = \kwundef$ and thus the abspec triggers UB.
Second, when $\powder = 1 \land \mres = \ready$, both implementation and abspec assign \code{1} to \code{r} and print \code{1};
the implementation decrements $\powder$ by \code{1} yielding \code{0} while
for \textcolor{blue}{\code{\GUARANTEE($\lambda$\res{}. \res{} == \kwemp \&\& r == 1)}}
the abspec updates $(\mres, \lres)$ to $(\fired, \kwemp)$, which is frame-preserving, and
\emph{chooses} $\kwemp$ for $\res$ to satisfy the postcondition and successfully subtract $\kwemp$ from $\lres$ yielding $\kwemp$;
finally both return the same value $\code{1}$ and establish the relational invariant with $\powder = 0 \land \mres = \fired$.
It is important to note that invariants relating implementations and abspecs like $(\powder = 1 \land \mres = \ready) \lor (\powder = 0 \land \mres = \fired)$ above do not appear in the abspecs, but only as a part of simulation proofs.

Finally, we can compose the abspecs to erase the specification parts:
\[
\begin{array}{@{}rl@{}}
&\beh{\spcmod{S_\Main \cup S_\Cannon}{(A_\Main,\mires_\Main)}{S_\Main} \link \spcmod{S_\Main \cup S_\Cannon}{(A_\Cannon,\mires_\Cannon)}{S_\Cannon}}\\
\subseteq & \beh{A_\Main \link A_\Cannon}
\end{array}
\]
We can prove this theorem, called \emph{spec erasure theorem}, as follows.
To \emph{discharge} the initial \ASSUME{} of $\Main.\main()$ (\ie to replace it with \kwskip),
we just need to choose an initial resource $\mires_\main$ to $\Main.\main()$, which will be $\ball$ here, and show that
$(i)$ it is consistent with the initial module-local resources (\ie \code{$\mires_\main$ + $\mires_\Main$ + $\mires_\Cannon$ != \kwundef{}})
and $(ii)$ it satisfies the precondition of $\Main.\main()$ (\ie \code{$\mires_\main$ == \ball}).
Then each remaining \textcolor{red}{\code{\ASSUME($Cond$)}} with a predicate $Cond$ on $\kwcanonpcm$ is discharged by the immediately preceding \textcolor{blue}{\code{\GUARANTEE($Cond$)}} with the same predicate.
To prove this, we first show that consistency of the whole resources (\ie those stored in all $\mres$ and $\lres$) is invariant:
the consistency holds initially because we have shown it by $(i)$ above,
and is preserved by \textcolor{blue}{\code{\GUARANTEE($Cond$)}}; \textcolor{red}{\code{\ASSUME($Cond$)}}
because the frame-preserving update via $\kwfpu$ preserves it by definition
and, by $(\star)$ above, the subtracted resource $\res$ in \GUARANTEE{} is immediately added back in \ASSUME{}.
Then we can complete the proof by discharging all the assumptions in \ASSUME{}, again by $(\star)$:
\textcolor{red}{\code{\kwassume($Cond$(\res))}} is discharged by \textcolor{blue}{\code{\kwguarantee($Cond$(\res))}},
and \textcolor{red}{\code{\kwassume(\mres{} + \lres{} != \kwundef)}} by the above invariant (\ie consistency of the whole resources).
Note that the spec erasure theorem holds in general among any compatible abspecs:
for example, even when ${\numfire = 2}$, the above erasure holds.

To conclude, the most important idea in \crems is
to give an illusion of passing logical information
via \kwchoose{} and \kwtake{} in an operational way.
In the next section, we will see how this powerful mechanism can be used
to model various logical features seamlessly.

%% in this section we have presented the key ideas of \crems using simple examples with a particular PCM and slightly informal definitions.
%% We will see formal and general definitions working for arbitrary PCMs in \Cref{sec:formal}.
%% \todo{say that via choose and take we can make illusion of logical data passing. we will see it various applications in the next section.}

%% \ASSUME{}s are discharged by the two matching \GUARANTEE{}
%% all remaining \ASSUME{} and \GUARANTEE{} are discharged by the following lemma:
%% for any predicate $Cond$ on $\kwcanonpcm$ and any program with a hole $K[-]$,
%% \[
%% \beh{K[\textcolor{blue}{\code{\GUARANTEE($Cond$)}}; \textcolor{red}{\code{\ASSUME($Cond$)}}]} \subseteq \beh{K[\kwskip]}
%% \]
%% \todo{fix the lemma statement}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

